Heuristics for Exact Nonnegative Matrix Factorization

The exact nonnegative matrix factorization (exact NMF) problem is the following: given an $m$-by-$n$ nonnegative matrix $X$ and a factorization rank $r$, find, if possible, an $m$-by-$r$ nonnegative matrix $W$ and an $r$-by-$n$ nonnegative matrix $H$ such that $X = WH$. In this paper, we propose two heuristics for exact NMF, one inspired from simulated annealing and the other from the greedy randomized adaptive search procedure. We show that these two heuristics are able to compute exact nonnegative factorizations for several classes of nonnegative matrices (namely, linear Euclidean distance matrices, slack matrices, unique-disjointness matrices, and randomly generated matrices) and as such demonstrate their superiority over standard multi-start strategies. We also consider a hybridization between these two heuristics that allows us to combine the advantages of both methods. Finally, we discuss the use of these heuristics to gain insight on the behavior of the nonnegative rank, i.e., the minimum factorization rank such that an exact NMF exists. In particular, we disprove a conjecture on the nonnegative rank of a Kronecker product, propose a new upper bound on the extension complexity of generic $n$-gons and conjecture the exact value of (i) the extension complexity of regular $n$-gons and (ii) the nonnegative rank of a submatrix of the slack matrix of the correlation polytope.

==> tables/file-table-LEDM32-rbr.tex <==
\begin{table}[h]
\begin{center}
\caption{Rank-by-Rank Heuristic on the LEDM32 for different values of $K$ and $N$.}
\begin{tabular}{|c||c|c|c|c|}
\hline
 & $K=1$ & $K=5$ & $K=10$ & $K=50$ \\
\hline
$N=10$  & 4/1000 (946.5)     & 1/1000 (3213.4)    & 0/1000 ($\sim$3.2) & 0/1000 ($\sim$3.8)  \\
$N=50$  & 4/1000 (838.3)     & 0/1000 ($\sim$3.8) & 0/1000 ($\sim$3.7) & 0/1000 ($\sim$5.1)  \\
$N=100$ & 0/1000 ($\sim$3.4) & 0/1000 ($\sim$4.7) & 0/1000 ($\sim$5)   & 0/1000 ($\sim$8.1)  \\
$N=500$ & 1/1000 (3408.5)    & 0/1000 ($\sim$4.5) & 0/1000 ($\sim$6.7) & 0/1000 ($\sim$24.5) \\
\hline
\end{tabular}
\label{table-LEDM32-rbr}
\end{center}
\end{table}


==> tables/file-table-final-sup.tex <==
\begin{table}[h]
\begin{center}
\caption{Final results.}
\begin{tabular}{|c||c|c|c|c|c|}
\hline
 & SA & RBR & Hybrid \\
\hline
LEDM64 & 0/100 ($\sim$44) & 0/100 ($\sim$7.7) & 0/100 ($\sim$44.5) \\
SM9 & 5/30 (78) & \textbf{7/10 (2.7)} & 7/10 (18.9) \\
SM10 & 2/100 (795.6) & \textbf{5/50 (30.2)} & 6/30 (81.5) \\
SM11 & 6/10 (26.5) & \textbf{8/30 (11)} & 7/10 (24) \\
SM12 & \textbf{10/10 (1.5)} & 10/10 (1.7) & 10/10 (1.7) \\
\hline
\end{tabular}
\label{finaltable}
\end{center}
\end{table}

==> tables/resultsGRASP-SA.tex <==
\newpage
\newgeometry{left=2cm,right=2cm,bottom=1.2cm,top=1cm}
\begin{table}[h] 
  \begin{center}
    \footnotesize 
    \begin{tabular}{|c|c|c||c|c|c|c|c|}
      \hline
					                                                & $m$ & $n$ & 0.5        & 0.9        & 0.99       & 0.9999 \\ 
      \hline  
      $M(i,j) = (i-j)^2$                                  & 6   & 6   & 1399(1399) & 1400(1400) & 1393(1393) & 1393(1393) \\
																									        & 8   & 8   & 0(721)     & 194(290)   & 232(232)   & 229(229)   \\
																									        & 12  & 12  &            &            &            &            \\
																									        & 16  & 16  &            &            &            &            \\
																										      & 32  & 32  &            &            &            &            \\
      % \hline  
      % $5 \times$ $M(i,j) = (a(i)-a(j))^2$                 & 7   & 7   &            &            &            &            \\
      % ($a \in \mathbb{R}^6$ uniform at random in $[0,1]$) &	    &     &            &            &            &            \\
      % Matrix 1                                            &	    &     &            &            & 0(748)     & 0(227)     \\
      % Matrix 2                                            &	    &     &            &            & 0(748)     &            \\
      % Matrix 3                                            &	    &     &            &            & 0(419)     &            \\
      % Matrix 4                                            &	    &     &            &            &            &            \\
      \hline  
      Slack Matrix 1 - Hexagon                            &	6   & 6   & 1400(1400) & 1400(1400) & 1399(1399) & 1400(1400) \\
      Slack Matrix 2 - Octagon                            &	8   & 8   & 1289(1289) & 1286(1286) & 1288(1288) & 1288(1288) \\
      Slack Matrix 3 - 16gon                              &	16  & 16  & 1071(1071) & 1071(1071) & 1071(1071) & 1071(1071) \\
      Slack Matrix 4 - Dodecahedron                       &	20  & 12  & 966(967)   & 963(967)   & 960(966)   & 965(966)   \\ 
      Slack Matrix 5 - 32gon                              &	32  & 32  & 823(843)   & 825(839)   & 814(833)   & 818(833)   \\
      Slack Matrix 6                                      &	    &     &            &            &            &            \\
      Slack Matrix 7                                      &	    &     &            &            &            &            \\
      Slack Matrix 8                                      &	    &     &            &            &            &            \\
      Slack Matrix 9                                      &	    &     &            &            &            &            \\
      Slack Matrix 10                                     &	    &     &            &            &            &            \\
      \hline 
      $10 \times$ Random Matrices                         & 50  & 50  &            &            &            &            \\
      ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &            &            &            &            \\
      0.1               																	&	    &     & 223(223)   & 226(226)   & 225(225)   & 225(225)   \\
      0.1             																		&	    &     & 226(226)   & 226(226)   & 225(225)   & 225(225)   \\
      0.3																									&	    &     & 215(215)   & 225(225)   & 227(227)   & 227(227)   \\
      0.3                                                 &	    &     & 227(227)   & 227(227)   & 227(227)   & 227(227)   \\
      0.5                                                 &	    &     &            &            &            &            \\
      0.5                                                 &	    &     &            &            &            &            \\
      0.7                                                 &	    &     &            &            &            &            \\
      0.7                                                 &	    &     &            &            &            &            \\
      0.9                                                 &	    &     &            &            &            &            \\
      0.9                                                 &	    &     &            &            &            &            \\
      \hline 
    \end{tabular}
    \scriptsize{\caption{\scriptsize Rank-by-Rank - Number of exact factorizations found during one hour (with the number of attempts in brackets).}}
    \label{results-onehour-grasp}
    \end{center}
  \end{table}




  \begin{table}[h!]
    \begin{center}
      \footnotesize 
      \begin{tabular}{|c|c|c||c|c|c|c|c|}
        \hline
					                                                  & $m$ & $n$ & 0.5         & 0.9         & 0.99       & 0.9999     \\ 
        \hline  
        $M(i,j) = (i-j)^2$                                  & 6   & 6   & 547(1325)   & 465(1094)   & 424(1072)  & 414(1061)  \\
																									          & 8   & 8   & 43(863)     & 49(622)     & 74(481)    & 76(450)    \\
																									          & 12  & 12  &             &             &            &            \\
																									          & 16  & 16  &             &             &            &            \\
																										        & 32  & 32  &             &             &            &            \\
        % \hline  
        % $5 \times$ $M(i,j) = (a(i)-a(j))^2$                 & 7   & 7   &             &             &            &            \\
        % ($a \in \mathbb{R}^6$ uniform at random in $[0,1]$) &	    &     &             &             &            &            \\
        % Matrix 1                                            &	    &     & 5(849)      & 19(726)     & 13(443)    & 7(65)      \\
        % Matrix 2                                            &	    &     & 0(868)      & 0(776)      & 1(377)     & 2(111)     \\
        % Matrix 3                                            &	    &     & 0(835)      & 0(740)      & 0(526)     & 0(130)     \\
        % Matrix 4                                            &	    &     & 50(849)     & 35(529)     & 73(380)    & 38(221)    \\
        \hline  
        Slack Matrix 1 - Hexagon                            &	6   & 6   & 1071(1679)  & 1022(1537)  & 837(1277)  & 793(1253)  \\
        Slack Matrix 2 - Octagon                            &	8   & 8   & 408(1561)   & 256(993)    & 274(1001)  & 263(995)   \\
        Slack Matrix 3 - 16gon                              &	16  & 16  & 6(857)      & 2(840)      & 3(810)     & 5(754)     \\
        Slack Matrix 4 - Dodecahedron                       &	20  & 12  &             &             &            &            \\
        Slack Matrix 5 - 32gon                              &	32  & 32  &             &             &            &            \\
        Slack Matrix 6                                      &	    &     &             &             &            &            \\
        Slack Matrix 7                                      &	    &     &             &             &            &            \\
        Slack Matrix 8                                      &	    &     &             &             &            &            \\
        Slack Matrix 9                                      &	    &     &             &             &            &            \\
        Slack Matrix 10                                     &	    &     &             &             &            &            \\
        \hline 
        $10 \times$ Random Matrices                         & 50  & 50  &             &             &            &            \\
        ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &             &             &            &            \\
        0.1               																	&	    &     & 1408(1458)  & 1408(1456)  & 1398(1449) & 1387(1428) \\
        0.1             																		&	    &     & 947(1458)   & 940(1454)   & 902(1399)  & 811(1063)  \\
        0.3																									&	    &     &             &             &            &            \\
        0.3                                                 &	    &     &             &             &            &            \\
        0.5                                                 &	    &     &             &             &            &            \\
        0.5                                                 &	    &     &             &             &            &            \\
        0.7                                                 &	    &     &             &             &            &            \\
        0.7                                                 &	    &     &             &             &            &            \\
        0.9                                                 &	    &     &             &             &            &            \\
        0.9                                                 &	    &     &             &             &            &            \\
        \hline 
      \end{tabular}  
      \caption{\scriptsize Simulated Annealing - Number of exact factorizations found during one hour (with the number of attempts in brackets).} 
      \label{results-onehour-sa-delta2}
  \end{center}
\end{table}

\newpage
\restoregeometry


==> tables/resultsInit.tex <==
\newpage
\newgeometry{left=2cm,right=2cm,bottom=1.2cm,top=1cm}
% \begin{table}[h] 
%   \begin{center}
%     \footnotesize 
%     \begin{tabular}{|c|c|c||c|c|c|c|c|c|c|}
%       \hline
% 					                                                & $m$ & $n$ & 0.001        & 0.005        &  0.01         & 0.05       & 0.1        & 1        & U[0,1]   \\ 
%       \hline   
%       $M(i,j) = (i-j)^2$                                  & 6   & 6   & 7/10 (3.4)   & 6/10 (3.6)   &  5/20 (4.4)   &    &    &  &  \\
% 																									        & 8   & 8   & 6/60 (7.2)   & 5/50 (6.4)   &  3/100 (6.9)  &    &    &  &  \\
% 																									        & 12  & 12  & 0/100 (11.8) & 0/100 (13.4) &  0/100 (13.1) &    &    &  &  \\
% 																									        & 16  & 16  & 0/100 (30.1) & 0/100 (32.8) &  0/100 (31.6) &    &    &  &  \\
%       \hline  
%       6-gon                                               &	6   & 6   & 10/10 (2.8)  & 10/10 (2.9)  &               &    &    &  &  \\
%       7-gon                                               &	7   & 7   & 10/10 (2.9)  & 10/10 (3.1)  &               &    &    &  &  \\
%       8-gon                                               &	8   & 8   & 5/10 (3.9)   & 9/20 (4.1)   &               &    &    &  &  \\
%       9-gon                                               &	9   & 9   & 8/20 (4.2)   & 6/10(3.9)    &               &    &    &  &  \\
%       16-gon                                              &	16  & 16  & 0/100 (5.7)  & 0/100 (5.9)  &               &    &    &  &  \\
%       32-gon                                              &	32  & 32  & 0/100 (17.2) & 0/100 (19.5) &               &    &    &  &  \\
%       Dodecahedron                                        &	20  & 12  & 2/100 (5.2)  & 1/100 (5.3)  &               &    &    &  &  \\
%       \hline 
%       $10 \times$ Random Matrices                         & 50  & 50  &              &              &               &    &    &  &  \\
%       ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &              &              &               &    &    &  &  \\
%       0.1               																	&	    &     & 10/10 (3.6)  & 10/10 (3.8)  &               &    &    &  &  \\
%       0.1             																		&	    &     & 10/10 (3.6)  & 10/10 (3.8)  &               &    &    &  &  \\
%       0.3																									&	    &     & 10/10 (3.6)  & 10/10 (3.8)  &               &    &    &  &  \\
%       0.3                                                 &	    &     & 10/10 (3.6)  & 10/10 (3.8)  &               &    &    &  &  \\
%       \hline 
%     \end{tabular}
%     \scriptsize{\caption{\scriptsize Comparisons between different types of initializations.}}
%     \label{results-onehour-grasp}
%   \end{center}
% \end{table}

\begin{table}[h] 
  \begin{center}
    \footnotesize 
    \begin{tabular}{|c|c|c||c|c|c|c|c|c|}
      \hline
					                                         & $m$ & $n$ & 0.0005       & 0.001        & 0.005        & 0.01         & 0.05         & U[0,1]       \\ 
      \hline   
      $M(i,j) = (i-j)^2$                           & 6   & 6   & 7/20 (4)     & 7/10 (3)     & 8/20 (3.7)   &              & 3/100 (4.4)  & 5/40 (4.4)   \\
																									 & 8   & 8   & 5/40 (5.2)   & 6/40 (5)     & 6/90 (5.6)   &              & 0/100 (4.9)  & 0/100 (5.1)  \\
																									 & 12  & 12  & 0/100 (9.7)  & 0/100 (7.9)  & 0/100 (7.8)  &              & 0/100 (7.8)  & 0/100 (8.2)  \\
																									 & 16  & 16  & 0/100 (21.4) & 0/100 (20.2) & 0/100 (18.9) & 0/100 (20.9) & 0/100 (17.2) & 0/100 (21)   \\
      \hline  
      6-gon                                        &	6  & 6   & 10/10 (2.7)  & 10/10 (2.5)  & 10/10 (2.5)  & 10/10 (2.5)  & 10/10 (2.5)  & 10/10 (2.4)  \\
      7-gon                                        &	7  & 7   & 10/10 (2.7)  & 10/10 (2.5)  & 10/10 (2.5)  & 10/10 (2.5)  & 9/10 (2.7)   & 9/10 (2.6)   \\
      8-gon                                        &	8  & 8   & 7/10 (3.3)   & 8/10 (2.9)   & 9/20 (3.6)   & 5/10 (3.5)   & 11/30 (3.8)  & 8/40 (4)     \\
      9-gon                                        &	9  & 9   & 7/10 (3.3)   & 5/10 (3.5)   & 8/10 (2.9)   & 7/10 (3.1)   & 5/20 (4.1)   & 5/10 (3.5)   \\
      16-gon                                       &	16 & 16  & 0/100 (4.9)  & 0/100 (4.7)  & 0/100 (4.7)  & 0/100 (4.7)  & 0/100 (4.7)  & 0/100 (4.9)  \\
      32-gon                                       &	32 & 32  & 0/100 (11.1) & 0/100 (10.9) & 0/100 (11.3) & 0/100 (11.9) & 0/100 (12.3) & 0/100 (17.3) \\
      Dodecahedron                                 &	20 & 12  & 0/100 (4.8)  & 0/100 (4.7)  & 0/100 (4.7)  & 1/100 (4.7)  & 0/100 (4.7)  & 0/100 (4.5)  \\
      \hline 
      $10 \times$ Random Matrices                  & 50  & 50  &              &              &              &              &              &              \\
      ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9) &	   &     &              &              &              &              &              &              \\
      0.1               													 &	   &     & 10/10 (3.6)  & 10/10 (2.9)  & 10/10 (2.9)  & 10/10 (2.9)  & 10/10 (2.9)  & 10/10 (2.7)  \\
      0.1             														 &	   &     &              &              &              &              &              &              \\
      0.3																					 &	   &     &              &              &              &              &              &              \\
      0.3                                          &	   &     &              &              &              &              &              &              \\
      \hline 
    \end{tabular}
    \scriptsize{\caption{\scriptsize Comparisons between different types of initializations.}}
    \label{results-onehour-grasp}
  \end{center}
\end{table}
  
\begin{table}[h] 
  \begin{center}
    \footnotesize 
    \begin{tabular}{|c|c|c||c|c|c|c|}
      \hline
					                                                & $m$ & $n$ & $crU=0$, $crV=0$ & $crU=0$, $crV=1$ &  $crU=1$, $crV=1$ & $crU=1$, $crV=0$ \\ 
      \hline   
      $M(i,j) = (i-j)^2$                                  & 6   & 6   & 0/100 (4.4)      & 0/100 (4.4)      & 0/100 (4.4)       & 0/100 (4.4)      \\
																									        & 8   & 8   & 0/100 (4.8)      & 0/100 (4.9)      & 0/100 (5)         & 0/100 (4.7)      \\
																									        & 12  & 12  & 0/100 (7)        & 0/100 (7.7)      & 0/100 (8.1)       & 0/100 (6.8)      \\
																									        & 16  & 16  & 0/100 (15.2)     & 0/100 (17.5)     & 0/100 (19.4)      & 0/100 (13.9)     \\
      \hline  
      6-gon                                               &	6   & 6   & 0/100 (4.4)      & 10/10 (2.4)      & 10/10 (2.4)       & 0/100 (4.4)      \\
      7-gon                                               &	7   & 7   & 0/100 (4.4)      & 1/100 (4.4)      & 2/100 (4.4)       & 0/100 (4.4)      \\
      8-gon                                               &	8   & 8   & 0/100 (4.4)      & 5/20 (3.9)       & 5/30 (4.1)        & 0/100 (4.4)      \\
      9-gon                                               &	9   & 9   & 0/100 (4.5)      & 7/80 (4.3)       & 1/100 (4.4)       & 0/100 (4.5)      \\
      16-gon                                              &	16  & 16  & 0/100 (4.6)      & 0/100 (4.6)      & 0/100 (4.7)       & 0/100 (4.6)      \\
      32-gon                                              &	32  & 32  & 0/100 (9.5)      & 0/100 (11.2)     & 0/100 (10.9)      & 0/100 (9.1)      \\
      Dodecahedron                                        &	20  & 12  & 0/100 (4.5)      & 0/100 (4.5)      & 0/100 (4.5)       & 0/100 (4.5)      \\
      \hline 
      $10 \times$ Random Matrices                         & 50  & 50  &                  &                  &                   &                  \\
      ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &                  &                  &                   &                  \\
      0.1               																	&	    &     & 10/10 (2.7)      & 10/10 (2.7)      & 10/10 (2.7)       & 10/10 (2.7)      \\
      0.1             																		&	    &     &                  &                  &                   &                  \\
      0.3																									&	    &     &                  &                  &                   &                  \\
      0.3                                                 &	    &     &                  &                  &                   &                  \\
      \hline 
    \end{tabular}
    \scriptsize{\caption{\scriptsize Comparisons between different types of initializations.}}
    \label{results-onehour-grasp}
    \end{center}
  \end{table}
\newpage
\restoregeometry

% \begin{table}[h] 
%   \begin{center}
%     \footnotesize 
%     \begin{tabular}{|c|c|c||c|c|c|c|c|c|c|}
%       \hline
% 					                                                & $m$ & $n$ & 0.001        & 0.005        &  0.01       & 0.05       & 0.1        & 1        & U[0,1]   \\ 
%       \hline   
%       $M(i,j) = (i-j)^2$                                  & 6   & 6   & 7/10 (3.4)   & 6/10 (3.6)   &  45(142)    & 14(129)    & 7(126)     & 16(129)  & 17(133)  \\
% 																									        & 8   & 8   & 6/60 (7.2)   & 5/50 (6.4)   &  0(77)      & 1(91)      & 0(89)      & 2(88)    & 2(88)    \\
% 																									        & 12  & 12  & 0/100 (11.8) & 0/100 (13.4) &  0(52)      & 0(51)      & 0(51)      & 0(43)    & 0(48)    \\
% 																									        & 16  & 16  & 0/100 (30.1) & 0/100 (32.8) &  0(18)      & 0(19)      & 0(21)      & 0(14)    & 0(19)    \\
%       \hline  
%       6-gon                                               &	6   & 6   & 10/10 (2.8)  & 10/10 (2.9)  &  215(215)   & 218(218)   & 219(219)   & 219(219) & 227(227) \\
%       7-gon                                               &	7   & 7   & 10/10 (2.9)  & 10/10 (3.1)  &  207(209)   & 191(204)   & 171(196)   & 176(198) & 176(203) \\
%       8-gon                                               &	8   & 8   & 5/10 (3.9)   & 9/20 (4.1)   &  90(160)    & 67(152)    & 46(144)    & 27(136)  & 34(142)  \\
%       9-gon                                               &	9   & 9   & 8/20 (4.2)   & 6/10(3.9)    &  78(153)    & 50(143)    & 54(145)    & 55(144)  & 39(142)  \\
%       16-gon                                              &	16  & 16  & 0/100 (5.7)  & 0/100 (5.9)  &  0(106)     & 0(108)     & 0(105)     & 0(91)    & 0(90)    \\
%       32-gon                                              &	32  & 32  & 0/100 (17.2) & 0/100 (19.5) &  0(33)      & 0(33)      & 0(31)      & 0(28)    & 0(22)    \\
%       Dodecahedron                                        &	20  & 12  & 2/100 (5.2)  & 1/100 (5.3)  &  2(117)     & 0(115)     & 0(117)     & 0(118)   & 0(123)   \\ 
%       \hline 
%       $10 \times$ Random Matrices                         & 50  & 50  &              &              &             &            &            &          &          \\
%       ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &              &              &             &            &            &          &          \\
%       0.1               																	&	    &     & 10/10 (3.6)  & 10/10 (3.8)  &  167(167)   & 170(170)   & 171(171)   & 173(173) & 196(196) \\
%       0.1             																		&	    &     & 10/10 (3.6)  & 10/10 (3.8)  &  169(169)   & 168(168)   & 171(171)   & 172(172) & 196(196) \\
%       0.3																									&	    &     & 10/10 (3.6)  & 10/10 (3.8)  &  171(171)   & 171(171)   & 171(171)   & 173(173) & 196(196) \\
%       0.3                                                 &	    &     & 10/10 (3.6)  & 10/10 (3.8)  &  171(171)   & 171(171)   & 171(171)   & 172(172) & 196(196) \\
%       \hline 
%     \end{tabular}
%     \scriptsize{\caption{\scriptsize Comparisons between different types of initializations.}}
%     \label{results-onehour-grasp}
%     \end{center}
%   \end{table}


==> tables/resultsInit2.tex <==
\newpage
\newgeometry{left=2cm,right=2cm,bottom=1.2cm,top=1cm}
\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & 0.0005 & 0.001 & 0.005 & 0.01 & 0.05 \\
\hline
 $EDMINT6$ & 6/40 (4.9) & 5/20 (4.5) & 5/20 (4.3) & 5/40 (4.7) & 6/90 (4.8) \\
 $EDMINT8$ & 1/100 (6.8) & 6/100 (7) & 2/100 (6.8) & 0/100 (6.7) & 0/100 (6.5) \\
 $EDMINT12$ & 0/100 (12.7) & 0/100 (10.8) & 0/100 (12.8) & 0/100 (12.1) & 0/100 (12.4) \\
 $hexagon$ & 9/10 (3) & 10/10 (2.9) & 10/10 (2.8) & 10/10 (2.8) & 10/10 (2.9) \\
 $7gon$ & 9/10 (3.1) & 10/10 (2.9) & 9/10 (3.1) & 10/10 (2.9) & 9/10 (3.1) \\
 $octagon$ & 5/20 (4.4) & 9/20 (4) & 8/20 (4.1) & 10/20 (3.9) & 8/20 (4.1) \\
 $9gon$ & 6/20 (4.4) & 6/30 (4.6) & 5/10 (4) & 8/20 (4.2) & 5/10 (4) \\
 $16gon$ & 0/100 (5.9) & 0/100 (5.8) & 0/100 (5.8) & 0/100 (5.7) & 0/100 (6.2) \\
 $dodecahedron$ & 2/100 (5.2) & 0/100 (5.2) & 0/100 (5.2) & 2/100 (5.2) & 1/100 (5.2) \\
 $RNDSP01_1$ & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.6) & 10/10 (3.7) \\
 $RNDSP01_2$ & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.6) \\
 $RNDSP03_1$ & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.7) \\
 $RNDSP03_2$ & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.6) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize dirichlet}}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & 0.0005 & 0.001 & 0.005 & 0.01 & 0.05 \\
\hline
 $EDMINT6$ & 6/20 (5) & 5/20 (4.4) & 6/30 (4.4) & 6/60 (5.1) & 5/80 (5.2) \\
 $EDMINT8$ & 5/40 (7.8) & 5/80 (7.4) & 0/100 (6.7) & 3/100 (6.9) & 0/100 (7.2) \\
 $EDMINT12$ & 0/100 (11.7) & 0/100 (12.5) & 0/100 (14.3) & 0/100 (12) & 0/100 (12.3) \\
 $hexagon$ & 10/10 (3.3) & 10/10 (2.9) & 10/10 (2.8) & 10/10 (2.8) & 10/10 (2.8) \\
 $7gon$ & 9/10 (3.4) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 7/10 (3.5) \\
 $octagon$ & 7/10 (3.8) & 7/20 (4.2) & 7/10 (3.5) & 6/10 (3.7) & 5/20 (4.4) \\
 $9gon$ & 8/20 (4.4) & 9/20 (4.1) & 7/20 (4.3) & 6/10 (3.8) & 6/20 (4.4) \\
 $16gon$ & 0/100 (6) & 0/100 (5.8) & 0/100 (5.9) & 0/100 (5.6) & 0/100 (5.8) \\
 $dodecahedron$ & 1/100 (5.3) & 2/100 (5.2) & 1/100 (5.2) & 1/100 (5.2) & 0/100 (5.2) \\
 $RNDSP01_1$ & 10/10 (4.7) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.6) & 10/10 (3.6) \\
 $RNDSP01_2$ & 10/10 (4.8) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.6) \\
 $RNDSP03_1$ & 10/10 (4.7) & 10/10 (3.7) & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.6) \\
 $RNDSP03_2$ & 10/10 (4.8) & 10/10 (3.7) & 10/10 (3.7) & 10/10 (3.6) & 10/10 (3.6) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize  dirichlet without NaN}}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & 0.0005 & 0.001 & 0.005 & 0.01 & 0.05 \\
\hline
 $EDMINT6$ & 8/30 (4.3) & 6/10 (3.6) & 5/10 (3.8) & 6/20 (4.2) & 5/60 (4.7) \\
 $EDMINT8$ & 3/100 (6.8) & 5/60 (7.2) & 6/80 (7.3) & 2/100 (7) & 1/100 (7.8) \\
 $EDMINT12$ & 0/100 (12.6) & 0/100 (12.3) & 0/100 (12.6) & 0/100 (12.9) & 0/100 (11.5) \\
 $hexagon$ & 10/10 (2.8) & 10/10 (2.8) & 10/10 (2.8) & 10/10 (2.8) & 10/10 (2.8) \\
 $7gon$ & 8/10 (3.3) & 10/10 (2.9) & 9/10 (3.1) & 10/10 (2.9) & 9/10 (3.1) \\
 $octagon$ & 5/20 (4.4) & 8/10 (3.3) & 6/10 (3.7) & 5/10 (3.9) & 7/10 (3.5) \\
 $9gon$ & 10/20 (4) & 5/10 (4) & 8/20 (4.2) & 5/10 (4) & 5/20 (4.5) \\
 $16gon$ & 0/100 (5.8) & 0/100 (5.6) & 0/100 (5.8) & 0/100 (5.5) & 0/100 (5.9) \\
 $dodecahedron$ & 2/100 (5.2) & 1/100 (5.2) & 1/100 (5.2) & 1/100 (5.2) & 1/100 (5.2) \\
 $RNDSP01_1$ & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) \\
 $RNDSP01_2$ & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) \\
 $RNDSP03_1$ & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) \\
 $RNDSP03_2$ & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize dirichlet with Uinit(Uinit$<$1e-6)=0 and Vinit(Vinit$<$1e-6)=0}}
\end{center}
\end{table}



\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & 0.0005 & 0.001 & 0.005 & 0.01 & 0.05 \\
\hline
 $EDMINT6$ & 5/10 (4.2) & 11/20 (3.8) & 5/10 (3.8) & 5/20 (4.5) & 5/100 (5.1) \\
 $EDMINT8$ & 6/20 (6.5) & 7/40 (6.8) & 4/100 (7.9) & 1/100 (6.6) & 0/100 (6.6) \\
 $EDMINT12$ & 0/100 (14) & 0/100 (12.7) & 0/100 (12.8) & 0/100 (14.6) & 0/100 (12.5) \\
 $hexagon$ & 10/10 (3.2) & 10/10 (2.9) & 10/10 (2.8) & 10/10 (2.8) & 10/10 (2.9) \\
 $7gon$ & 10/10 (3.2) & 10/10 (2.9) & 10/10 (2.9) & 9/10 (3.1) & 8/10 (3.3) \\
 $octagon$ & 7/10 (3.8) & 7/10 (3.5) & 10/20 (3.9) & 10/20 (4) & 5/20 (4.4) \\
 $9gon$ & 6/10 (4) & 11/20 (3.9) & 5/10 (4) & 10/20 (4) & 8/20 (4.3) \\
 $16gon$ & 0/100 (5.8) & 0/100 (5.8) & 0/100 (5.7) & 0/100 (5.7) & 0/100 (5.9) \\
 $dodecahedron$ & 2/100 (5.3) & 0/100 (5.2) & 1/100 (5.2) & 1/100 (5.2) & 0/100 (5.2) \\
 $RNDSP01_1$ & 10/10 (4.7) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.7) \\
 $RNDSP01_2$ & 10/10 (4.7) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.7) \\
 $RNDSP03_1$ & 10/10 (4.7) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.6) \\
 $RNDSP03_2$ & 10/10 (4.7) & 10/10 (3.6) & 10/10 (3.6) & 10/10 (3.7) & 10/10 (3.7) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize dirichlet with Uinit(Uinit$<$1e-6)=0 and Vinit(Vinit$<$1e-6)=0, without NaN}}
\end{center}
\end{table}

\newpage


\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & crU=0,crV=0 & crU=0,crV=1 & crU=1,crV=1 & crU=1,crV=0 \\
\hline
 $EDMINT6$ & 0/100 (4.8) & 0/100 (4.8) & 0/100 (4.8) & 0/100 (4.8) \\
 $EDMINT8$ & 0/100 (5.7) & 0/100 (5.9) & 0/100 (6.2) & 0/100 (5.7) \\
 $EDMINT12$ & 0/100 (10.7) & 0/100 (12.6) & 0/100 (13.4) & 0/100 (9.3) \\
 $hexagon$ & 0/100 (4.8) & 10/10 (2.8) & 10/10 (2.8) & 0/100 (4.8) \\
 $7gon$ & 0/100 (4.8) & 5/60 (4.7) & 2/100 (4.8) & 0/100 (4.8) \\
 $octagon$ & 0/100 (4.8) & 5/10 (3.9) & 5/10 (3.8) & 0/100 (4.8) \\
 $9gon$ & 0/100 (4.9) & 3/100 (4.9) & 2/100 (4.9) & 0/100 (4.9) \\
 $16gon$ & 0/100 (5.2) & 0/100 (5.5) & 0/100 (5.7) & 0/100 (5.3) \\
 $dodecahedron$ & 0/100 (5) & 0/100 (5.1) & 0/100 (5) & 0/100 (5) \\
 $RNDSP01_1$ & 10/10 (3.2) & 10/10 (3.4) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP01_2$ & 10/10 (3.2) & 10/10 (3.5) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP03_1$ & 10/10 (3.2) & 10/10 (3.3) & 10/10 (3.3) & 10/10 (3.2) \\
 $RNDSP03_2$ & 10/10 (3.2) & 10/10 (3.3) & 10/10 (3.2) & 10/10 (3.2) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize sparse}}
\end{center}
\end{table}



\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & crU=0,crV=0 & crU=0,crV=1 & crU=1,crV=1 & crU=1,crV=0 \\
\hline
 $EDMINT6$ & 0/100 (4.8) & 0/100 (4.8) & 0/100 (4.8) & 0/100 (4.8) \\
 $EDMINT8$ & 0/100 (5.5) & 0/100 (6) & 0/100 (6.3) & 0/100 (5.2) \\
 $EDMINT12$ & 0/100 (10.5) & 0/100 (13.2) & 0/100 (11.7) & 0/100 (9.8) \\
 $hexagon$ & 0/100 (4.8) & 10/10 (2.8) & 10/10 (2.8) & 0/100 (4.8) \\
 $7gon$ & 0/100 (4.8) & 1/100 (4.8) & 4/100 (4.8) & 0/100 (4.8) \\
 $octagon$ & 0/100 (4.8) & 5/40 (4.7) & 8/50 (4.5) & 0/100 (4.8) \\
 $9gon$ & 0/100 (4.9) & 1/100 (4.9) & 1/100 (4.9) & 0/100 (4.9) \\
 $16gon$ & 0/100 (5.2) & 0/100 (5.7) & 0/100 (5.6) & 0/100 (5.2) \\
 $dodecahedron$ & 0/100 (5) & 0/100 (5.1) & 0/100 (5.1) & 0/100 (5) \\
 $RNDSP01_1$ & 10/10 (3.3) & 10/10 (3.3) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP01_2$ & 10/10 (3.2) & 10/10 (3.3) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP03_1$ & 10/10 (3.3) & 10/10 (3.3) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP03_2$ & 10/10 (3.2) & 10/10 (3.4) & 10/10 (3.2) & 10/10 (3.2) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize sparse + 1e-16}}
\end{center}
\end{table}



\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & crU=0,crV=0 & crU=0,crV=1 & crU=1,crV=1 & crU=1,crV=0 \\
\hline
 $EDMINT6$ & 0/100 (4.8) & 0/100 (4.8) & 0/100 (4.8) & 0/100 (4.8) \\
 $EDMINT8$ & 0/100 (5.6) & 0/100 (6.5) & 0/100 (6.3) & 0/100 (5.4) \\
 $EDMINT12$ & 0/100 (9.2) & 0/100 (11.4) & 0/100 (11.4) & 0/100 (9.6) \\
 $hexagon$ & 0/100 (4.8) & 10/10 (2.8) & 10/10 (2.7) & 0/100 (4.8) \\
 $7gon$ & 0/100 (4.8) & 3/100 (4.8) & 4/100 (4.7) & 0/100 (4.8) \\
 $octagon$ & 0/100 (4.8) & 5/40 (4.6) & 5/20 (4.3) & 0/100 (4.8) \\
 $9gon$ & 0/100 (4.9) & 1/100 (4.9) & 4/100 (4.8) & 0/100 (4.9) \\
 $16gon$ & 0/100 (5.1) & 0/100 (5.5) & 0/100 (5.6) & 0/100 (5.2) \\
 $dodecahedron$ & 0/100 (5) & 0/100 (5) & 0/100 (5) & 0/100 (5) \\
 $RNDSP01_1$ & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP01_2$ & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP03_1$ & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) \\
 $RNDSP03_2$ & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) & 10/10 (3.2) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize sparse + 1e-10}}
\end{center}
\end{table}
\newpage
\restoregeometry


==> tables/resultsInit3.tex <==
\newpage
\newgeometry{left=2cm,right=2cm,bottom=1.2cm,top=1cm}
\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & crU=0,crV=0 & crU=0,crV=1 & crU=1,crV=1 & crU=1,crV=0 \\
\hline
 $EDMINT6$ & 6/60 (4.3) & 8/10 (2.9) & 6/10 (3.3) & 5/20 (4) \\
 $EDMINT8$ & 3/100 (5.3) & 6/50 (5.8) & 6/20 (4.3) & 2/100 (5.3) \\
 $EDMINT12$ & 0/100 (9.9) & 0/100 (9.5) & 0/100 (9.6) & 0/100 (10.5) \\
 $hexagon$ & 10/10 (2.5) & 10/10 (2.5) & 10/10 (2.5) & 10/10 (2.5) \\
 $7gon$ & 9/10 (2.7) & 10/10 (2.5) & 10/10 (2.5) & 8/10 (2.9) \\
 $octagon$ & 9/20 (3.7) & 6/10 (3.4) & 8/10 (3) & 7/20 (3.9) \\
 $9gon$ & 7/20 (3.9) & 7/10 (3.2) & 7/10 (3.2) & 7/20 (4) \\
 $16gon$ & 0/100 (5.1) & 0/100 (5) & 0/100 (5) & 0/100 (4.8) \\
 $dodecahedron$ & 0/100 (4.7) & 2/100 (4.7) & 1/100 (4.7) & 0/100 (4.7) \\
 $RNDSP01_1$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
 $RNDSP01_2$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
 $RNDSP03_1$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
 $RNDSP03_2$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize One element by row (column or line)}}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & crU=0,crV=0 & crU=0,crV=1 & crU=1,crV=1 & crU=1,crV=0 \\
\hline
 $EDMINT6$ & 5/10 (3.5) & 6/30 (4.5) & 8/20 (3.7) & 8/30 (4) \\
 $EDMINT8$ & 2/100 (6) & 2/100 (6.2) & 3/100 (6.6) & 3/100 (6.3) \\
 $EDMINT12$ & 0/100 (9.7) & 0/100 (11.1) & 0/100 (10.9) & 0/100 (10.7) \\
 $hexagon$ & 10/10 (2.5) & 10/10 (2.5) & 10/10 (2.5) & 10/10 (2.5) \\
 $7gon$ & 7/10 (3.1) & 9/10 (2.7) & 10/10 (2.6) & 9/10 (2.7) \\
 $octagon$ & 10/20 (3.6) & 5/10 (3.6) & 7/10 (3.2) & 6/10 (3.4) \\
 $9gon$ & 8/10 (3) & 5/30 (4.3) & 6/10 (3.4) & 7/20 (3.9) \\
 $16gon$ & 0/100 (5.1) & 0/100 (5.1) & 0/100 (5) & 0/100 (5) \\
 $dodecahedron$ & 5/90 (4.6) & 4/100 (4.6) & 5/80 (4.6) & 5/50 (4.5) \\
 $RNDSP01_1$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
 $RNDSP01_2$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
 $RNDSP03_1$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.9) \\
 $RNDSP03_2$ & 10/10 (2.9) & 10/10 (3) & 10/10 (2.9) & 10/10 (2.9) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize Two elements by row (column or line)}}
\end{center}
\end{table}


\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 & crU=0,crV=0 & crU=0,crV=1 & crU=1,crV=1 & crU=1,crV=0 \\
\hline
 $EDMINT6$ & 7/30 (4.4) & 6/20 (4.3) & 6/20 (5) & 5/50 (4.7) \\
 $EDMINT8$ & 2/100 (8.1) & 0/100 (7.1) & 3/100 (7.5) & 5/60 (10.1) \\
 $EDMINT12$ & 0/100 (15.9) & 0/100 (14.1) & 0/100 (14.3) & 0/100 (15.4) \\
 $hexagon$ & 10/10 (2.9) & 10/10 (2.9) & 10/10 (2.8) & 10/10 (2.8) \\
 $7gon$ & 10/10 (2.9) & 8/10 (3.3) & 8/10 (3.3) & 9/10 (3.1) \\
 $octagon$ & 5/20 (4.4) & 6/40 (4.6) & 6/20 (4.3) & 7/20 (4.2) \\
 $9gon$ & 8/30 (4.9) & 9/40 (4.6) & 6/20 (4.4) & 6/20 (4.6) \\
 $16gon$ & 0/100 (6.5) & 0/100 (6.3) & 0/100 (6.7) & 0/100 (6.2) \\
 $dodecahedron$ & 4/100 (5.1) & 5/70 (5) & 0/100 (5.2) & 0/100 (5.2) \\
 $RNDSP01_1$ & 10/10 (3.5) & 10/10 (3.5) & 10/10 (3.4) & 10/10 (3.4) \\
 $RNDSP01_2$ & 10/10 (3.5) & 10/10 (3.5) & 10/10 (3.4) & 10/10 (3.4) \\
 $RNDSP03_1$ & 10/10 (3.5) & 10/10 (3.5) & 10/10 (3.5) & 10/10 (3.4) \\
 $RNDSP03_2$ & 10/10 (3.5) & 10/10 (3.5) & 10/10 (3.5) & 10/10 (3.4) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize Three elements by row (column or line)}}
\end{center}
\end{table}
\newpage
\restoregeometry


==> tables/resultsMS1MS2.tex <==
\newpage
\newgeometry{left=2cm,right=2cm,bottom=1.2cm,top=1cm}
\begin{table}[h] 
  \begin{center}
    \footnotesize 
    \begin{tabular}{|c|c|c||c|c|c|c|c|}
    \hline
					                                              & $m$ & $n$ & ANLS & MU & A-MU & HALS & A-HALS \\ 
    \hline  
    $M(i,j) = (i-j)^2$                                  & 6   & 6   & 10(894) & 12(638) & 19(625) & 4(851) & 4(851) \\ 
																									      & 8   & 8   & 0(719) & 0(527) & 2(536) & 0(816) & 0(816) \\ 
																									      & 12  & 12  &        &    &      &      &     \\ 
																									      & 16  & 16  &        &    &      &      &     \\ 
																										    & 32  & 32  &        &    &      &      &     \\ 
    % \hline  
    % $5 \times$ $M(i,j) = (a(i)-a(j))^2$                 & 7   & 7   &      &    &      &      &     \\ 
    % ($a \in \mathbb{R}^6$ uniform at random in $[0,1]$) &	    &     &      &    &      &      &     \\
    % Matrix 1                                            &	    &     & 13(595) & 2(422) & 2(373) & 8(597)  & 8(601)  \\
    % Matrix 2                                            &	    &     & 6(560)  & 0(438) & 0(436) & 2(320)  & 2(319)  \\
    % Matrix 3                                            &	    &     & 0(496)  & 0(296) & 0(287) & 0(375)  & 0(381)  \\
    % Matrix 4                                            &	    &     & 21(735) & 0(542) &        & 23(657) & 26(661) \\
    \hline  
    Slack Matrix 1 - Hexagon                            &	6   & 6   & 2(1014) & 63(332) & 86(354) & 60(926) & 60(926) \\ 
    Slack Matrix 2 - Octagon                            &	8   & 8   & 1(921)  & 34(169) & 44(239) & 24(908) & 23(907) \\ 
    Slack Matrix 3 - 16gon                              &	16  & 16  & 0(779)  & 0(475)  & 0(518)  & 0(849)  & 0(851)  \\ 
    Slack Matrix 4 - Dodecahedron                       &	20  & 12  & 1(890)  & 6(729)  & 4(836)  & 0(896)  & 0(896)  \\ 
    Slack Matrix 5 - 32gon                              &	32  & 32  &         &         &         &         &         \\ 
    Slack Matrix 6                                      &	    &     &         &         &         &         &         \\ 
    Slack Matrix 7                                      &	    &     &         &         &         &         &         \\ 
    Slack Matrix 8                                      &	    &     &         &         &         &         &         \\ 
    Slack Matrix 9                                      &	    &     &         &         &         &         &         \\ 
    Slack Matrix 10                                     &	    &     &         &         &         &         &         \\ 
    \hline 
    $10 \times$ Random Matrices                         & 50  & 50  &            &    &      &      &     \\ 
    ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &            &    &      &      &     \\
    0.1	(pc-isieres)																		&	    &     & 850(1315)  & 84(130) & 136(233) & 1526(1656) & 1524(1655) \\
    0.1	(pc-isieres)																		&	    &     & 701(1236)  & 63(183) & 104(266) & 1139(1417) & 1132(1412) \\

    0.3																									&	    &     & 1659(1723) & 50(53)  & 86(90)   & 1787(1787) & 1786(1786) \\
    0.3                                                 &     &     & 1731(1759) & 46(46)  & 80(80)   & 1787(1787) & 1786(1786) \\
    0.5 (pc-mons)                                       &	    &     & 1621(1687) & 3(19)   & 30(30)   & 1755(1755) & 1752(1752) \\
    0.5 (pc-isieres)                                    &	    &     & 1691(1740) & 38(38)  & 68(68)   & 1787(1787) & 1787(1787) \\
    0.7 (pc-isieres)                                    &	    &     & 1643(1715) & 27(27)  & 47(47)   & 1787(1787) & 1786(1786) \\
    0.7 (pc-isieres)                                    &	    &     & 1688(1738) & 31(31)  & 56(56)   & 1787(1787) & 1787(1787) \\
    0.9 (pc-isieres)                                    &	    &     & 1572(1680) & 23(23)  & 41(41)   & 1787(1787) & 1787(1787) \\
    \hline  
    \end{tabular}
    \scriptsize{\caption{\scriptsize Multi-Start 1 - Number of exact factorizations found during one hour (with the number of attempts in brackets).}}
    \label{results-onehour-ms1}
    \end{center}
  \end{table}




  \begin{table}[h!]
    \begin{center}
      \footnotesize 
      \begin{tabular}{|c|c|c||c|c|c|c|c|}
        \hline
                                              & $m$ & $n$ & ANLS   & MU      & A-MU     & HALS     & A-HALS   \\ 
        \hline  
        $M(i,j) = (i-j)^2$                                  & 6   & 6   & 52(93) & 1(583)  & 6(539)   & 108(510) & 114(518) \\ 
														                  & 8   & 8   & 1(46)  & 0(474)  & 1(462)   & 7(422)   & 5(424)   \\ 
														                  & 12  & 12  & 0(63)  & 0(317)  & 0(317)   & 1(324)   & 0(325)   \\ 
														                  & 16  & 16  &        &         &          &          &          \\ 
															                & 32  & 32  &        &         &          &          &          \\ 
        % \hline  
        % $5 \times$ $M(i,j) = (a(i)-a(j))^2$                 & 7   & 7   &        &         &          &          &          \\ 
        % ($a \in \mathbb{R}^6$ uniform at random in $[0,1]$) &	    &     &        &         &          &          &          \\
        % Matrix 1                                            &	    &     & 17(67) & 1(431)  & 1(444)   & 11(369)  & 12(365)  \\
        % Matrix 2                                            &	    &     & 4(58)  & 0(469)  & 0(450)   & 0(300)   & 0(295)   \\
        % Matrix 3                                            &	    &     & 0(53)  & 0(349)  & 0(350)   & 0(272)   & 0(272)   \\
        % Matrix 4                                            &	    &     & 20(74) & 0(487)  & 3(417)   & 7(414)   & 9(413)   \\
        \hline  
        Slack Matrix 1 - Hexagon                            &	6   & 6   & 0(93)  & 56(331) & 93(296)  & 676(676) & 675(675) \\ 
        Slack Matrix 2 - Octagon                            &	8   & 8   & 7(83)  & 27(246) & 42(197)  & 454(593) & 452(590) \\ 
        Slack Matrix 3 - 16gon                              &	16  & 16  & 0(53)  & 0(400)  & 0(402)   & 0(414)   & 0(401)   \\ 
        Slack Matrix 4 - Dodecahedron                       &	20  & 12  & 0(45)  & 5(546)  & 6(515)   & 13(422)  & 12(413)  \\ 
        Slack Matrix 5 - 32gon                              &	32  & 32  &        &         &          &          &          \\ 
        Slack Matrix 6                                      &	    &     &        &         &          &          &          \\
        Slack Matrix 7                                      &	    &     &        &         &          &          &          \\
        Slack Matrix 8                                      &	    &     &        &         &          &          &          \\
        Slack Matrix 9                                      &	    &     &        &         &          &          &          \\
        Slack Matrix 10                                     &	    &     &        &         &          &          &          \\
        \hline 
        $10 \times$ Random Matrices                         & 50  & 50  &        &         &          &          &          \\
        ($2 \times$ Density 0.1, 0.3, 0.5, 0.7, 0.9)        &	    &     &        &         &          &          &          \\
        0.1               																	&	    &     & 44(44) & 75(100) & 116(116) & 431(431) & 435(435) \\
        0.1             																		&	    &     & 45(45) & 58(124) & 100(101) & 449(449) & 443(443) \\
        0.3																									&	    &     & 44(44) & 47(48)  & 76(76)   & 446(446) & 443(443) \\
        0.3                                                 &     &     & 41(41) & 43(43)  & 70(70)   & 439(439) & 431(431) \\
        0.5                                                 &	    &     & 37(37) & 32(33)  & 49(50)   & 389(389) & 402(402) \\
        0.5                                                 &	    &     & 44(44) & 36(37)  & 61(61)   & 447(447) & 447(447) \\
        0.7                                                 &	    &     & 46(46) & 26(26)  & 44(44)   & 445(445) & 444(444) \\
        0.7                                                 &	    &     & 45(45) & 31(31)  & 51(51)   & 445(445) & 438(438) \\
        0.9                                                 &	    &     & 49(49) & 22(22)  & 37(37)   & 440(440) & 437(437) \\
        0.9                                                 &	    &     & 49(49) & 20(21)  & 34(34)   & 443(443) & 440(440) \\
        \hline  
      \end{tabular}
      \caption{\scriptsize Multi-Start 2 - Number of exact factorizations found during one hour (with the number of attempts in brackets).} 
      \label{results-onehour-ms2}
  \end{center}
\end{table}

\newpage
\restoregeometry


==> tables/results_table2.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|}
\hline
 & ANLS & MU & A-MU & HALS & A-HALS \\
\hline
LEDM6 &  & 0/100 (7.1) & 0/100 (6.3) & 8/10 (2.9) & 8/10 (3) \\
LEDM8 &  & 0/100 (8.9) & 0/100 (6.3) & 5/20 (5.3) & 6/30 (5.3) \\
LEDM12 &  &  & 0/100 (10.9) & 0/100 (9.6) & 0/100 (9.2) \\
LEDM16 &  &  & 0/100 (21.9) & 0/100 (24.7) & 0/100 (22.1) \\
LEDM32 &  &  & 0/100 (60.5) & 0/100 (54.8) & 0/100 (48.5) \\
SM1 &  &  & 0/100 (4.3) & 10/10 (2.5) & 10/10 (2.5) \\
SM2 &  &  & 0/100 (4.3) & 10/10 (2.6) & 10/10 (2.6) \\
SM3 &  &  & 0/100 (5.5) & 13/20 (3.3) & 13/20 (3.3) \\
SM4 &  &  & 3/100 (6.4) & 8/10 (3) & 8/10 (3) \\
SM5 &  &  & 0/100 (7.5) & 0/100 (4.9) & 0/100 (4.8) \\
SM6 &  &  & 0/100 (22.5) & 0/100 (11) & 0/100 (10.7) \\
SM7 &  &  & 0/100 (4.5) & 1/100 (4.7) & 1/100 (4.7) \\
SM8 &  &  & 0/100 (4.6) & 0/100 (4.9) & 0/100 (4.9) \\
UDISJ4 &  &  & 0/100 (4.3) & 10/10 (2.7) & 10/10 (2.7) \\
UDISJ5 &  &  & 0/100 (4.6) & 5/10 (4.3) & 5/10 (4.2) \\
UDISJ6 &  &  & 0/100 (8.2) & 2/100 (6.7) & 3/100 (6.8) \\
RND1 &  &  & 6/10 (10.1) & 10/10 (2.9) & 10/10 (2.8) \\
RND2 &  &  & 10/10 (10.9) & 10/10 (2.9) & 10/10 (2.9) \\
RND3 &  &  & 10/10 (21.6) & 10/10 (2.9) & 10/10 (2.9) \\
RND4 &  &  & 10/10 (23.2) & 10/10 (2.9) & 10/10 (2.9) \\
\hline
\end{tabular}
\scriptsize{\caption{\scriptsize initsparse11-ms2}}
\end{center}
\end{table}

